Impact of the Dresden-II and COHERENT neutrino scattering data on neutrino electromagnetic properties and electroweak physics

Coherent elastic neutrino-nucleus scattering (CE$\nu$NS) represents a powerful tool to investigate key electroweak physics parameters and neutrino properties since its first observation in 2017 by the COHERENT experiment exploiting the spallation neutron source at Oak Ridge National Laboratory. In light of the recent detection of such a process with antineutrinos produced by the Dresden-II reactor scattering off a germanium detector, we revisit the limits so far set on the neutrino magnetic moments, charge radii and millicharges as well as on the weak mixing angle. In order to do so, we also include the contribution of elastic neutrino-electron scattering, whose effect becomes non negligible in some beyond the Standard Model theories. By using different hypotheses for the germanium quenching factor and the reactor antineutrino flux, we provide a measurement of the weak mixing angle at the low-energy scale of the Dresden-II reactor experiment and, thanks to a combined analysis with the latest cesium iodide and argon data set released by the COHERENT Collaboration, we deliver updated limits for the neutrino electromagnetic properties. Interestingly, we are able to set a new best upper limit on the electron neutrino charge radius and significantly improve the other CE$\nu$NS-related limits on the neutrino electric charge and magnetic moment.

==> tables/tab22-ech5-tot.tex <==
\begin{tabular}{ccccc}
&
$1\sigma$
&
$90\%$
&
$2\sigma$
%&
%$99\%$
&
$3\sigma$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (HMVE-Fef CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -7.2 , 7.5 )\times10^{ -12 }$
&
$( -9.2 , 9.4 )\times10^{ -12 }$
&
$( -1.0 , 1.0 )\times10^{ -11 }$
%&
%$( -1.2 , 1.2 )\times10^{ -11 }$
&
$( -1.2 , 1.3 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.3 , 2.2 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 7.3 \times10^{ -12 }$
&
$< 9.4 \times10^{ -12 }$
&
$< 1.0 \times10^{ -11 }$
%&
%$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 7.4 \times10^{ -12 }$
&
$< 9.4 \times10^{ -12 }$
&
$< 1.0 \times10^{ -11 }$
%&
%$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.3 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (HMK-Fef CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -6.6 , 6.8 )\times10^{ -12 }$
&
$( -8.5 , 8.6 )\times10^{ -12 }$
&
$( -9.3 , 9.5 )\times10^{ -12 }$
%&
%$( -1.0 , 1.1 )\times10^{ -11 }$
&
$( -1.1 , 1.2 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.3 , 2.3 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 6.6 \times10^{ -12 }$
&
$< 8.6 \times10^{ -12 }$
&
$< 9.4 \times10^{ -12 }$
%&
%$< 1.1 \times10^{ -11 }$
&
$< 1.1 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 6.7 \times10^{ -12 }$
&
$< 8.6 \times10^{ -12 }$
&
$< 9.4 \times10^{ -12 }$
%&
%$< 1.1 \times10^{ -11 }$
&
$< 1.1 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.3 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (EFK-Fef CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -7.4 , 7.6 )\times10^{ -12 }$
&
$( -9.0 , 9.4 )\times10^{ -12 }$
&
$( -1.0 , 1.0 )\times10^{ -11 }$
%&
%$( -1.1 , 1.1 )\times10^{ -11 }$
&
$( -1.2 , 1.2 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.3 , 2.2 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 7.5 \times10^{ -12 }$
&
$< 9.3 \times10^{ -12 }$
&
$< 1.0 \times10^{ -11 }$
%&
%$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 7.4 \times10^{ -12 }$
&
$< 9.3 \times10^{ -12 }$
&
$< 1.0 \times10^{ -11 }$
%&
%$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.3 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (HMVE-YBe CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -1.1 , 1.1 )\times10^{ -11 }$
&
$( -1.2 , 1.2 )\times10^{ -11 }$
&
$( -1.3 , 1.3 )\times10^{ -11 }$
%&
%$( -1.4 , 1.4 )\times10^{ -11 }$
&
$( -1.5 , 1.5 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.2 , 2.2 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
%&
%$< 1.4 \times10^{ -11 }$
&
$< 1.5 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
%&
%$< 1.4 \times10^{ -11 }$
&
$< 1.5 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.3 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (HMK-YBe CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -9.8 , 10.2 )\times10^{ -12 }$
&
$( -1.1 , 1.1 )\times10^{ -11 }$
&
$( -1.2 , 1.2 )\times10^{ -11 }$
%&
%$( -1.3 , 1.3 )\times10^{ -11 }$
&
$( -1.4 , 1.4 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.3 , 2.2 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 1.0 \times10^{ -11 }$
&
$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
%&
%$< 1.3 \times10^{ -11 }$
&
$< 1.4 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 1.0 \times10^{ -11 }$
&
$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
%&
%$< 1.3 \times10^{ -11 }$
&
$< 1.4 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.2 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\multicolumn{5}{c}{\bf CsI (CEvNS+ES) + Ar (CEvNS) + Dresden-II (EFK-YBe CEvNS+ES)}
\\
%\hline
$q_{\nu_{ee}}$
&
$( -1.0 , 1.1 )\times10^{ -11 }$
&
$( -1.2 , 1.2 )\times10^{ -11 }$
&
$( -1.3 , 1.3 )\times10^{ -11 }$
%&
%$( -1.4 , 1.4 )\times10^{ -11 }$
&
$( -1.4 , 1.4 )\times10^{ -11 }$
\\
%\hline
$q_{\nu_{\mu\mu}}$
&
$( -1.2 , 1.2 )\times10^{ -10 }$
&
$( -1.9 , 1.9 )\times10^{ -10 }$
&
$( -2.3 , 2.3 )\times10^{ -10 }$
%&
%$( -2.8 , 2.8 )\times10^{ -10 }$
&
$( -3.2 , 3.2 )\times10^{ -10 }$
\\
%\hline
$|q_{\nu_{e\mu}}|$
&
$< 1.1 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
%&
%$< 1.4 \times10^{ -11 }$
&
$< 1.4 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{e\tau}}|$
&
$< 1.0 \times10^{ -11 }$
&
$< 1.2 \times10^{ -11 }$
&
$< 1.3 \times10^{ -11 }$
%&
%$< 1.4 \times10^{ -11 }$
&
$< 1.4 \times10^{ -11 }$
\\
%\hline
$|q_{\nu_{\mu\tau}}|$
&
$< 1.2 \times10^{ -10 }$
&
$< 1.9 \times10^{ -10 }$
&
$< 2.3 \times10^{ -10 }$
%&
%$< 2.8 \times10^{ -10 }$
&
$< 3.2 \times10^{ -10 }$
\\
\hline
\end{tabular}

